AIT* and EIT*: Asymmetric bidirectional sampling-based path planning

Optimal path planning is the problem of finding a valid sequence of states between a start and goal that optimizes an objective. Informed path planning algorithms order their search with problem-specific knowledge expressed as heuristics and can be orders of magnitude more efficient than uninformed algorithms. Heuristics are most effective when they are both accurate and computationally inexpensive to evaluate, but these are often conflicting characteristics. This makes the selection of appropriate heuristics difficult for many problems. This paper presents two almost-surely asymptotically optimal sampling-based path planning algorithms to address this challenge, Adaptively Informed Trees (AIT*) and Effort Informed Trees (EIT*). These algorithms use an asymmetric bidirectional search in which both searches continuously inform each other. This allows AIT* and EIT* to improve planning performance by simultaneously calculating and exploiting increasingly accurate, problem-specific heuristics. The benefits of AIT* and EIT* relative to other sampling-based algorithms are demonstrated on twelve problems in abstract, robotic, and biomedical domains optimizing path length and obstacle clearance. The experiments show that AIT* and EIT* outperform other algorithms on problems optimizing obstacle clearance, where a priori cost heuristics are often ineffective, and still perform well on problems minimizing path length, where such heuristics are often effective.

==> figures/3-algorithms/3-1-adaptively-informed-trees/heuristics/combined_figure.tex <==
\begin{figure}
  \begin{center}
    Path length\vphantom{Obstacle clearance}
  \end{center}%
  \vspace{-0.8em}
  \begin{subfigure}[t]{0.49\columnwidth}
    \input{figures/3-algorithms/3-1-adaptively-informed-trees/heuristics/a-priori-heuristic}%
    \caption{Euclidean cost heuristic}%
    \label{fig:euclidean-heuristic}
  \end{subfigure}%
  \hfill%
  \begin{subfigure}[t]{0.49\columnwidth}
    \input{figures/3-algorithms/3-1-adaptively-informed-trees/heuristics/adaptive-heuristic}%
    \caption{Problem-specific cost heu\-ristic}%
    \label{fig:adaptive-heuristic}
  \end{subfigure}%
  \caption{This figure illustrates the benefits of using an adaptive heuristic over the Euclidean heuristic when optimizing path length. The start and goal are represented by a black dot~(\tikzinlinestart) and  circle~(\tikzinlinegoal), respectively. A selection of sampled states are represented by small black dots~(\tikzinlinestate). The state space obstacle is indicated with a gray rectangle~(\tikzinlineobstacle). According to the Euclidean heuristic, the green and red edges are equally promising~(\,\protect\tikz[baseline]{\protect\draw[forward edge, espgreen, yshift = 0.25em] (0,0) -- (1.1em, 0);}~\( + \)~\protect\tikz[baseline]{\protect\draw[forward edge, espgreen, dotted, yshift = 0.25em] (0,0) -- (1.1em, 0);}~\( = \) \,\protect\tikz[baseline]{\protect\draw[forward edge, espred, yshift = 0.25em] (0,0) -- (1.1em, 0);}~\( + \)~\protect\tikz[baseline]{\protect\draw[forward edge, espred, dotted, yshift = 0.25em] (0,0) -- (1.1em, 0);}\,), even though the red edge leads to a dead end~(\subref{fig:euclidean-heuristic}). According to the adaptive heuristic, the green edge is more promising than the red~(\,\protect\tikz[baseline]{\protect\draw[forward edge, espgreen, yshift = 0.25em] (0,0) -- (1.1em, 0);}~\( + \)~\protect\tikz[baseline]{\protect\draw[forward edge, espgreen, dashed, yshift = 0.25em] (0,0) -- (1.1em, 0);}~\( < \)~\,\protect\tikz[baseline]{\protect\draw[forward edge, espred, yshift = 0.25em] (0,0) -- (1.1em, 0);}~\( + \)~\protect\tikz[baseline]{\protect\draw[forward edge, espred, dashed, yshift = 0.25em] (0,0) -- (1.1em, 0);}\,), which can lead the search around the obstacle without evaluating many unnecessary edges~(\subref{fig:adaptive-heuristic}).}%
  \label{fig:benefits-of-adaptive-heuristics}
\end{figure}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../../../../main"
%%% End:


==> preamble/algorithm-operations.tex <==
\newcommand{\updateheuristic}[1]{\texttt{update\_heuristic}\left(#1\right)}
\newcommand{\updateheuristics}[1]{\texttt{update\_heuristics}\left(#1\right)}
\newcommand{\mpsupdatestate}[1]{\texttt{update\_state}\left(#1\right)}
\newcommand{\popbest}[1]{\texttt{get\_best}\left(#1\right)}
\newcommand{\lowerbound}[1]{\texttt{lower\_bound}\left(#1\right)}
\newcommand{\isvalid}[1]{\texttt{collision\_free}\left(#1\right)}
\newcommand{\couldbevalid}[1]{\texttt{no\_sparse\_collisions\_detected}\left(#1\right)}
\newcommand{\mpsexpand}[1]{\texttt{expand}\left(#1\right)}
\newcommand{\mpsfparent}[1]{\texttt{parent}_{\mathcal{F}}\left(#1\right)}
\newcommand{\mpsrparent}[1]{\texttt{parent}_{\mathcal{R}}\left(#1\right)}
\newcommand{\mpsfchildren}[1]{\texttt{children}_{\mathcal{F}}\left(#1\right)}
\newcommand{\mpsrchildren}[1]{\texttt{children}_{\mathcal{R}}\left(#1\right)}
\newcommand{\mpssample}[1]{\texttt{sample}\left(#1\right)}
\newcommand{\mpsprune}[1]{\texttt{prune}\left(#1, c_{\mathrm{current}}\right)}
\newcommand{\mpsneighbors}[1]{\texttt{neighbors}\left(#1\right)}
\newcommand{\mpsnearest}[1]{\texttt{nearest}\left(#1, r \text{ or } k\right)}

==> preamble/mpsmiscellaneous.tex <==
% The acronym package makes sure every acronym is expanded at least once.
\usepackage{acronym}

\makeatletter
%A definite article (lower case) that is present for the full phrase but absent for the acronym
\newcommand{\dac}[1]{%
  \expandafter\ifx\csname AC@#1\endcsname\AC@used
    \acs{#1}%
  \else
    the \acf{#1}\acused{#1}%
  \fi
}
%The same as above but upper case.
\newcommand{\Dac}[1]{%
  \expandafter\ifx\csname AC@#1\endcsname\AC@used
    \acs{#1}%
  \else
    The \acf{#1}\acused{#1}%
  \fi
}
%A expansion-appropriate citation to an acronym.
\newcommand{\accite}[2]{%
  \expandafter\ifx\csname AC@#1\endcsname\AC@used
    \acs{#1} \citep{#2}%Easy-peezy.
  \else
%    \acf{#1}\acused{#1} \citep{#2}%If you're using [] citations
   \acl{#1}\acused{#1} \citep[\acs{#1};][]{#2}%If you're using () citations
  \fi
}
\makeatother

% The enumitem package let's us modify lists and add inline lists.
\usepackage[inline,shortlabels]{enumitem}

==> preamble/mpsnotation.tex <==
\usepackage{etoolbox}

% Constants
\newcommand{\ee}[1]{\mathrm{e}^{\ifblank{#1}{}{#1}}}

% Relationship symbols
\newcommand{\defeq}{\vcentcolon=}

% Measures
\newcommand{\lebesgue}[1]{\lambda{\left(\ifblank{#1}{\:\cdot\:}{#1}\right)}}

% Evaluation functions
\newcommand{\gtstandalone}{g_{\mathcal{T}}}
\newcommand{\gt}[1]{\gtstandalone\left(#1\right)}
\newcommand{\ghatstandalone}{\widehat{g}}
\newcommand{\ghat}[1]{\ghatstandalone\left(#1\right)}
\newcommand{\chatstandalone}{\widehat{c}}
\newcommand{\chat}[2]{\chatstandalone\left(#1, #2\right)}
\newcommand{\ctruestandalone}{c}
\newcommand{\ctrue}[2]{\ctruestandalone\left(#1, #2\right)}
\newcommand{\hhatstandalone}{\widehat{h}}
\newcommand{\hhat}[1]{\hhatstandalone\left(#1\right)}
\newcommand{\fhat}[1]{\widehat{f}\ifblank{#1}{}{\left(#1\right)}}

% States
\newcommand{\mpsstatespace}{X}
\newcommand{\mpssampledstates}{X_{\mathrm{sampled}}}
\newcommand{\mpsvalidstates}{X_{\mathrm{valid}}}
\newcommand{\mpsinvalidstates}{X_{\mathrm{invalid}}}

\newcommand{\mpsstate}{\bm{\mathrm{x}}}
\newcommand{\mpsstartstate}{\bm{\mathrm{x}}_{\mathrm{start}}}
\newcommand{\mpsgoalstate}{\bm{\mathrm{x}}_{\mathrm{goal}}}
\newcommand{\mpsgoalstates}{X_\mathrm{goal}}
\newcommand{\mpssourcestate}{\bm{\mathrm{x}}_{\mathrm{s}}}
\newcommand{\mpstargetstate}{\bm{\mathrm{x}}_{\mathrm{t}}}

\newcommand{\mpsinformedset}{X_\mathrm{informed}}

\newcommand{\sspace}{X}
\newcommand{\ssampled}{X_{\mathrm{sampled}}}
\newcommand{\sfree}{X_{\mathrm{free}}}
\newcommand{\sinformed}{X_{\fhatstandalone}}
\newcommand{\sobs}{X_{\mathrm{obs}}}
\newcommand{\sunconnected}{X_{\mathrm{unconnected}}}
\newcommand{\sstart}{\bm{\mathrm{x}}_{\mathrm{init}}}
\newcommand{\sgoal}{\bm{\mathrm{x}}_{\mathrm{goal}}}
\newcommand{\sgoals}{X_{\mathrm{goal}}}
\newcommand{\sany}{\bm{\mathrm{x}}}
\newcommand{\snum}[1]{\bm{\mathrm{x}}_{#1}}
\newcommand{\sparent}{\bm{\mathrm{x}}_{\mathrm{p}}}
\newcommand{\schild}{\bm{\mathrm{x}}_{\mathrm{c}}}
\newcommand{\ssource}{\bm{\mathrm{x}}_{\mathrm{s}}}
\newcommand{\starget}{\bm{\mathrm{x}}_{\mathrm{t}}}

% Edges
\newcommand{\eany}{\bm{\mathrm{e}}}

% Paths
\newcommand{\spath}{\sigma}
\newcommand{\fpath}{\sigma_{\mathrm{feasible}}}
\newcommand{\opath}{\sigma^{*}}
\newcommand{\spaths}{\Sigma}
\newcommand{\fpaths}{\Sigma_{\mathrm{feasible}}}
\newcommand{\opaths}{\Sigma_{*}}

% Search
\newcommand{\stree}{\mathcal{T}}
\newcommand{\svertices}{V}
\newcommand{\sedges}{E}
\newcommand{\sedgequeue}{\mathcal{Q}_{\mathrm{E}}}
\newcommand{\svertexqueue}{\mathcal{Q}_{\mathrm{V}}}
\newcommand{\sopen}{\mathtt{OPEN}}

\newcommand{\mpsopen}{\mathtt{OPEN}}
\newcommand{\mpsclosed}{\mathtt{CLOSED}}

% Algorithm
\newcommand{\sset}{\leftarrow{}}
\newcommand{\ssetinsert}{\xleftarrow{\scriptscriptstyle +}}
\newcommand{\ssetremove}{\xleftarrow{\scriptscriptstyle -}}

==> preamble/mpspdfpc.tex <==
% pdfpc commands \usepackage[absolute,overlay]{textpos} % Required for textblock* % Command for including a movie that fills the frame. % % Arguments:
%
%   [optional]: movie-options, seperated by &
%       Supported options: loop, start=N, end=N, autostart
%   Default: autostart&loop
%
%   1. Movie file
%   2. Poster image
%   3. Any text on the slide, or nothing (e.g. {})
%
% Example:
%   \fullframemovie[loop&autostart]{apollo17.avi}{apollo17.jpg}{\copyrightText{Apollo 17, NASA}}
%
\newcommand{\fullframemovie}[4][autostart&loop]
{
    {
        \setbeamercolor{background canvas}{bg=black}
        % To make this work for both horizontally filled and vertically filled images, we create an absolutely
        % positioned textblock* that we force to be the width of the slide.
        % we then place it at (0,0), and then create a box inside of it to ensure that it's always 95% of the vertical
        % height of the frame.  Once we have created an absolutely positioned and sized box, it doesn't matter what
        % goes inside -- it will always be vertically and horizontally centered
        \frame[plain]{%
            \begin{textblock*}{\paperwidth}(0\paperwidth,0\paperheight)%
            \centering%
            \vbox to 0.95\paperheight {%
                \vfil{%
                    \href{run:#2?autostart&#1}{\includegraphics[width=\paperwidth,height=0.95\paperheight,keepaspectratio]{#3}}%
                }%
                \vfil%
            }%
            \end{textblock*}%
            #4%
        }
    }
}

% Command for including a movie inline.
%
% Arguments:
%
%   [optional]: movie-options, seperated by &
%       Supported options: loop, start=N, end=N, autostart
%   Default: autostart&loop
%
%   1. Movie file
%   2. Poster image
%   3. size command, such as width=\textwidth
%
% Example:
%   \inlinemovie[loop&autostart&start=5&stop=12]{apollo17.avi}{apollo17.jpg}{height=0.7\textheight}
%
\newcommand{\inlinemovie}[4][autostart&loop]
{
    \href{run:#2?#1}{\includegraphics[#4]{#3}}
}


% Command for acknowleding copyrights.
%
% Produces small text on the right side of the screen, useful for
% stating copyright or other small notes in movies or images
%
% Arguments:
%
%   [optional]: text color
%       Default: white
%
%   1. Text to be displayed
%
% Example:
%   \copyrighttext{Full frame image of: Apollo 17, NASA}
%
\newcommand{\copyrighttext}[2][white]{%
 \begin{textblock*}{\paperwidth}(0\paperwidth,0.97\paperheight)%
    \hfill\textcolor{#1}{\tiny#2}\hspace{20pt}
  \end{textblock*}
}

% Command to include an image that covers the whole frame and shows the whole image.
%
% Produces a slide that contains a full frame image. Scales down the image
% to fit if the aspect ratio of the slide does not match the image.
%
% Arguments:
%
%   [optional]: color of text on page
%       Default: white
%
%   1. Path to image file
%   2. Any additional content on the frame
%
% Example:
%   \fullframeimagezoomed{apollo17.jpg}{\copyrightText{Full frame image of: Apollo 17, NASA}}
%
\newcommand{\fullframeimage}[3][white]
{
    {
        \setbeamercolor{normal text}{bg=black,fg=#1}

        % To make this work for both horizontally filled and vertically filled images, we create an absolutely
        % positioned textblock* that we force to be the width of the slide.
        % we then place it at (0,0), and then create a box inside of it to ensure that it's always 95% of the vertical
        % height of the frame.  Once we have created an absolutely positioned and sized box, it doesn't matter what
        % goes inside -- it will always be vertically and horizontally centered
        \frame{
            \begin{textblock*}{\paperwidth}(0\paperwidth,0\paperheight)
            \centering
            \vbox to 0.95\paperheight {
                \vfil{
                    \includegraphics[width=\paperwidth,height=0.95\paperheight,keepaspectratio]{#2}
                }
                \vfil
            }
            \end{textblock*}
            #3
        }
    }
}

% Command to include an image that covers the whole frame and zooms in if the aspect ratio of the image and frame don't match.
%
% Produces a slide that contains a full frame image.  If the aspect ratio
% of the image does not match the slide, it crops the image.
%
% Arguments:
%
%   [optional]: color of text on page
%       Default: black
%
%   1. Path to image file
%   2. Any additional content on the frame
%
% Example:
%   \fullframeimagezoomed{apollo17.jpg}{\copyrightText{Full frame image of: Apollo 17, NASA}}
%
\newcommand{\fullframeimagezoomed}[3][black]
{
    {
        \usebackgroundtemplate{\includegraphics[height=\paperheight]{#2}}
        \setbeamercolor{normal text}{bg=black,fg=#1}
        \frame{
            #3
        }
    }
}

==> preamble/mpspreamble.tex <==
% MIT License

% Copyright (c) 2017 Marlin Strub

% Permission is hereby granted, free of charge, to any person obtaining a copy
% of this software and associated documentation files (the "Software"), to deal
% in the Software without restriction, including without limitation the rights
% to use, copy, modify, merge, publish, distribute, sublicense, and/or sell
% copies of the Software, and to permit persons to whom the Software is
% furnished to do so, subject to the following conditions:

% The above copyright notice and this permission notice shall be included in all
% copies or substantial portions of the Software.

% THE SOFTWARE IS PROVIDED "AS IS", WITHOUT WARRANTY OF ANY KIND, EXPRESS OR
% IMPLIED, INCLUDING BUT NOT LIMITED TO THE WARRANTIES OF MERCHANTABILITY,
% FITNESS FOR A PARTICULAR PURPOSE AND NONINFRINGEMENT. IN NO EVENT SHALL THE
% AUTHORS OR COPYRIGHT HOLDERS BE LIABLE FOR ANY CLAIM, DAMAGES OR OTHER
% LIABILITY, WHETHER IN AN ACTION OF CONTRACT, TORT OR OTHERWISE, ARISING FROM,
% OUT OF OR IN CONNECTION WITH THE SOFTWARE OR THE USE OR OTHER DEALINGS IN THE
% SOFTWARE.

% Encoding
\usepackage[utf8]{inputenc}
\usepackage[T1]{fontenc}

% Babel for hyphenation rules
\usepackage[english]{babel}

% Use microtype
\usepackage{microtype}

% AMS Math
\usepackage{
  amsfonts,
  amsmath,
  amssymb,
  amsthm,
  bm,
  mathtools
}

% The mathtools and etoolbox packages.
\usepackage{
  etoolbox,
  mathtools
}

% We can now use referenced environemnts (such as align) everywhere and only the
% labels of referenced equations will be printed. Manual tags (\tag{...}) will
% always be printed.
\mathtoolsset{showonlyrefs,showmanualtags}

% Mathic takes care of italic correction in math mode.
\mathtoolsset{mathic}

% Paired Delimiters (uses mathtools and etoolbox)
% Sets (typeset as \set*{ x \in X \given Y })
\providecommand\given{}
\newcommand\SetSymbol[1][]{%
  \nonscript\:#1\vert%
  \allowbreak%
  \nonscript\:%
  \mathopen{}}
\DeclarePairedDelimiterX\set[1]{\{}{\}}{%
  \renewcommand\given{\SetSymbol[\delimsize]}%
  \ifblank{#1}{\:\cdots\:}{#1}
}

% Absolute values
\DeclarePairedDelimiterX{\abs}[1]{\vert}{\vert}{
  \ifblank{#1}{\:\cdot\:}{#1}
}

% Norms (typeset as \norm*{ x } or \lnorm*{ })
\DeclarePairedDelimiterX{\norm}[1]{\lVert}{\rVert}{
  \ifblank{#1}{\:\cdot\:}{#1}
}
\DeclarePairedDelimiterXPP{\lnorm}[1]{}{\lVert}{\rVert}{_{2}}{
  \ifblank{#1}{\:\cdot\:}{#1}
}
\DeclarePairedDelimiterXPP{\infnorm}[1]{}{\lVert}{\rVert}{_{\infty}}{
  \ifblank{#1}{\:\cdot\:}{#1}
}
\DeclarePairedDelimiterXPP{\pnorm}[2]{}{\lVert}{\rVert}{
  \ifblank{#2}{_{p}}{_{#2}}}{
  \ifblank{#1}{\:\cdot\:}{#1}
}

% Inner products (typeset as \inner*{ x } or \inner*{})
\DeclarePairedDelimiterX{\inner}[2]{\langle}{\rangle}{
  \ifblank{#1}{\:\cdot\:}{#1},\ifblank{#2}{\:\cdot\:}{#2}
}

% Probabilities (typeset as \prob*{ x \in X \given Y } or \prob*{})
\DeclarePairedDelimiterXPP{\prob}[1]{\mathbb{P}}{[}{]}{}{
  \renewcommand\given{\nonscript\:\delimsize\vert\nonscript\:\mathopen{}}
  \ifblank{#1}{\:\cdot\:}{#1}
}

% Expected values (typeset as \expv*{ X \given Y } or \expv*{})
\DeclarePairedDelimiterXPP{\expv}[1]{\mathbb{E}}{[}{]}{}{
  \renewcommand\given{\nonscript\:\delimsize\vert\nonscript\:\mathopen{}}
  \ifblank{#1}{\:\cdot\:}{#1}
}

% Theorems and definitions
% \newtheoremstyle{mpsdefinition}{2pt plus 2pt minus 0pt}{2pt plus 2pt minus 0pt}{\itshape}{0pt}{\bfseries}{.}{ }{\thmname{#1}\thmnumber{ #2}\thmnote{ \normalfont(#3)}}%
% \newtheorem{definition}{Definition}
% \theoremstyle{plain}
% \newtheorem{theorem}{Theorem}
% \theoremstyle{definition}
% \newtheorem{example}{Example}

% Source code
\usepackage{listings}

% Algorithms
\usepackage[linesnumbered,vlined,ruled,commentsnumbered]{algorithm2e}
\SetVlineSkip{0.4em}% Sets the skip after the small horizontal lines of control blocks.
\DontPrintSemicolon% The semicolon is just unnecessary clutter.
\SetKwIF{If}{ElseIf}{Else}{if}{}{else if}{else}{endif}% Really no need to print 'then'.
\SetAlgoSkip{}% Saves some whitespace in some cases.
\SetAlCapHSkip{0cm}% Zero indent for algrithm titles.

% Captions and subfigures
\usepackage{caption}
\usepackage{subcaption}
\usepackage{graphicx}
\usepackage{adjustbox}

% Graphics
\usepackage{tikz}
	\usetikzlibrary{calc,positioning}
	\tikzset{>=latex}
\usepackage{pgfplots, pgfplotstable}
\usepgfplotslibrary{statistics,fillbetween}
  \pgfplotsset{
    compat=1.15,
    mps basic/.style={
      xlabel near ticks,
      xlabel style={font=\footnotesize},
      ylabel near ticks,
      ylabel style={font=\footnotesize},
      xmajorgrids,
      major x grid style={dotted},
      ymajorgrids,
      major y grid style={dotted},
      tick label style={font=\footnotesize}
    },
    mps scientific x/.style={
      x tick label style={
        /pgf/number format/sci
      }
    },
    mps scientific y/.style={
      y tick label style={
        /pgf/number format/sci
      }
    },
    mps fixed x/.style={
      x tick label style={
        /pgf/number format/.cd,
        fixed,
        fixed zerofill,
        precision=6,
        /tikz/.cd
      }
    },
    mps fixed y/.style={
      y tick label style={
        /pgf/number format/.cd,
        fixed,
        fixed zerofill,
        precision=6,
        /tikz/.cd
      }
    }
  }

% pdfpc commands \usepackage[absolute,overlay]{textpos} % Required for textblock* % Command for including a movie that fills the frame. % % Arguments:
%
%   [optional]: movie-options, seperated by &
%       Supported options: loop, start=N, end=N, autostart
%   Default: autostart&loop
%
%   1. Movie file
%   2. Poster image
%   3. Any text on the slide, or nothing (e.g. {})
%
% Example:
%   \fullframemovie[loop&autostart]{apollo17.avi}{apollo17.jpg}{\copyrightText{Apollo 17, NASA}}
%
\newcommand{\fullframemovie}[4][autostart&loop]
{
    {
        \setbeamercolor{background canvas}{bg=black}
        % To make this work for both horizontally filled and vertically filled images, we create an absolutely
        % positioned textblock* that we force to be the width of the slide.
        % we then place it at (0,0), and then create a box inside of it to ensure that it's always 95% of the vertical
        % height of the frame.  Once we have created an absolutely positioned and sized box, it doesn't matter what
        % goes inside -- it will always be vertically and horizontally centered
        \frame[plain]{%
            \begin{textblock*}{\paperwidth}(0\paperwidth,0\paperheight)%
            \centering%
            \vbox to 0.95\paperheight {%
                \vfil{%
                    \href{run:#2?autostart&#1}{\includegraphics[width=\paperwidth,height=0.95\paperheight,keepaspectratio]{#3}}%
                }%
                \vfil%
            }%
            \end{textblock*}%
            #4%
        }
    }
}

% Command for including a movie inline.
%
% Arguments:
%
%   [optional]: movie-options, seperated by &
%       Supported options: loop, start=N, end=N, autostart
%   Default: autostart&loop
%
%   1. Movie file
%   2. Poster image
%   3. size command, such as width=\textwidth
%
% Example:
%   \inlinemovie[loop&autostart&start=5&stop=12]{apollo17.avi}{apollo17.jpg}{height=0.7\textheight}
%
\newcommand{\inlinemovie}[4][autostart&loop]
{
    \href{run:#2?#1}{\includegraphics[#4]{#3}}
}


% Command for acknowleding copyrights.
%
% Produces small text on the right side of the screen, useful for
% stating copyright or other small notes in movies or images
%
% Arguments:
%
%   [optional]: text color
%       Default: white
%
%   1. Text to be displayed
%
% Example:
%   \copyrighttext{Full frame image of: Apollo 17, NASA}
%
\newcommand{\copyrighttext}[2][white]{%
 \begin{textblock*}{\paperwidth}(0\paperwidth,0.97\paperheight)%
    \hfill\textcolor{#1}{\tiny#2}\hspace{20pt}
  \end{textblock*}
}

% Command to include an image that covers the whole frame and shows the whole image.
%
% Produces a slide that contains a full frame image. Scales down the image
% to fit if the aspect ratio of the slide does not match the image.
%
% Arguments:
%
%   [optional]: color of text on page
%       Default: white
%
%   1. Path to image file
%   2. Any additional content on the frame
%
% Example:
%   \fullframeimagezoomed{apollo17.jpg}{\copyrightText{Full frame image of: Apollo 17, NASA}}
%
\newcommand{\fullframeimage}[3][white]
{
    {
        \setbeamercolor{normal text}{bg=black,fg=#1}

        % To make this work for both horizontally filled and vertically filled images, we create an absolutely
        % positioned textblock* that we force to be the width of the slide.
        % we then place it at (0,0), and then create a box inside of it to ensure that it's always 95% of the vertical
        % height of the frame.  Once we have created an absolutely positioned and sized box, it doesn't matter what
        % goes inside -- it will always be vertically and horizontally centered
        \frame{
            \begin{textblock*}{\paperwidth}(0\paperwidth,0\paperheight)
            \centering
            \vbox to 0.95\paperheight {
                \vfil{
                    \includegraphics[width=\paperwidth,height=0.95\paperheight,keepaspectratio]{#2}
                }
                \vfil
            }
            \end{textblock*}
            #3
        }
    }
}

% Command to include an image that covers the whole frame and zooms in if the aspect ratio of the image and frame don't match.
%
% Produces a slide that contains a full frame image.  If the aspect ratio
% of the image does not match the slide, it crops the image.
%
% Arguments:
%
%   [optional]: color of text on page
%       Default: black
%
%   1. Path to image file
%   2. Any additional content on the frame
%
% Example:
%   \fullframeimagezoomed{apollo17.jpg}{\copyrightText{Full frame image of: Apollo 17, NASA}}
%
\newcommand{\fullframeimagezoomed}[3][black]
{
    {
        \usebackgroundtemplate{\includegraphics[height=\paperheight]{#2}}
        \setbeamercolor{normal text}{bg=black,fg=#1}
        \frame{
            #3
        }
    }
}

% Clickable references
% \usepackage[hidelinks]{hyperref}
